TraF-Align: Trajectory-aware Feature Alignment for Asynchronous Multi-agent Perception

Cooperative perception presents significant potential for enhancing the sensing capabilities of individual vehicles, however, inter-agent latency remains a critical challenge. Latencies cause misalignments in both spatial and semantic features, complicating the fusion of real-time observations from the ego vehicle with delayed data from others. To address these issues, we propose TraF-Align, a novel framework that learns the flow path of features by predicting the feature-level trajectory of objects from past observations up to the ego vehicle's current time. By generating temporally ordered sampling points along these paths, TraF-Align directs attention from the current-time query to relevant historical features along each trajectory, supporting the reconstruction of current-time features and promoting semantic interaction across multiple frames. This approach corrects spatial misalignment and ensures semantic consistency across agents, effectively compensating for motion and achieving coherent feature fusion. Experiments on two real-world datasets, V2V4Real and DAIR-V2X-Seq, show that TraF-Align sets a new benchmark for asynchronous cooperative perception.

==> sec/5_Conclusions.tex <==
\section{Conclusion}
\label{sec:conclusion}
Deploying LiDARs at urban intersections holds great promise for providing top-view perception services to intelligent vehicles.
%
However, 3D object detection suffers considerable challenges in point cloud quality, including \textbf{a)} reduced point cloud density and inadequate point cloud completeness due to the sensor's elevated installation heights, expansive coverage areas, and associated high costs, and \textbf{b)} diminished signal-to-noise ratio arising from the fixed viewpoint, resulting in a dramatic imbalance between background and object data.
%
We observe that roadside LiDARs offer a stable viewpoint and long-term observation capabilities, eliminating the need for frame-to-frame alignment. This allows us to effortlessly separate foreground and background based on extensive observations, achieving a lightweight 3D object detection method using multi-frame point cloud sequences.


==> table/ablation/pr_curve/frame_label_1.tex <==
\definecolor{mycolor1}{rgb}{0.00000,0.65000,0.85000}% 更明亮的蓝色
\definecolor{mycolor2}{rgb}{0.95000,0.60000,0.25000}% 明亮的橙色
\definecolor{mycolor3}{rgb}{0.97000,0.82000,0.35000}% 温暖的黄色
\definecolor{mycolor4}{rgb}{0.60000,0.30000,0.75000}% 鲜艳的紫色
\definecolor{mycolor5}{rgb}{0,0.6,0.1}% 深绿
\definecolor{mycolor6}{rgb}{0.45000,0.85000,0.95000}% 鲜艳的天蓝色
\definecolor{mycolor7}{rgb}{0.75000,0.20000,0.35000}% 明亮的粉红色
\definecolor{mycolor8}{rgb}{0.8,0.6,0.6}% 柔和的粉色
\definecolor{mycolor9}{rgb}{0.4,0.7,0.9}% 明亮的天蓝色
\definecolor{mycolor10}{rgb}{0.7,0.6,0.4}% 明亮的黄绿色
\definecolor{mycolor11}{rgb}{0.9,0.8,0.3}% 明亮的黄绿色
\definecolor{mycolor12}{rgb}{0.5,0.4,0.7}% 鲜艳的紫色
\definecolor{mycolor13}{rgb}{0.6,0.3,0.2}% 鲜艳的橙色
\definecolor{mycolor14}{rgb}{0.9,0.6,0.4}% 明亮的橙色
\definecolor{mycolor15}{rgb}{0.3,0.7,0.8}% 明亮的蓝绿色

\begin{tikzpicture}[font=\sffamily\scriptsize]
\node[draw=white,outer sep=0.5pt,inner sep=0pt] at (0,0) 
{
    \renewcommand{\arraystretch}{1.25} 
    \setlength{\tabcolsep}{2pt} % 设置列间距为 x pt
     \begin{tabular}{cccccccccccccc}
     \ref{prcurve_nofusion}&Single Agent &
     \ref{frame_1_1} & 1+1&\ref{frame_4_1} & 4+1 &
     \ref{frame_4_2} & 4+2 & \ref{frame_4_4} & 4+4 \\
    \end{tabular}
    };
\end{tikzpicture}
